First Experiences With Validating and Using the Cray Power Management Database Tool

In October 2013 CSCS installed the first hybrid Cray XC-30 system, dubbed Piz Daint. This system features the power management database (PMDB), that was recently introduced by Cray to collect detailed power consumption information in a non-intrusive manner. Power measurements are taken on each node, with additional measurements for the Aries network and blowers, and recorded in a database. This enables fine-grained reporting of power consumption that is not possible with external power meters, and is useful to both application developers and facility operators. This paper will show how benchmarks of representative applications at CSCS were used to validate the PMDB on Piz Daint. Furthermore we will elaborate, with the well-known HPL benchmark serving as prototypical application, on how the PMDB streamlines the tuning for optimal power efficiency in production, which lead to Piz Daint being recognised as the most energy efficient petascale supercomputer presently in operation.

==> cp2k.tex <==
\subsection{CP2K}
CP2K is a molecular dynamics code that performs atomistic and molecular simulations of solid state, liquid, molecular, and biological systems using different methods such as DFT using a mixed Gaussian and plane waves approach (GPW) and classical pair and many-body potentials. It uses a wide rango of computational kernels such as ense linear algebra (Cholesky, DGEMM, diagonalization), spase linear algebra (Matrix-Matrix and Matrix Vector multiplications), FFT, Time Integration and hemical Kernels. However, a single kernel does not dominates and the scaling ranges from $O(N)$ to $O(N^5)$.\\
For this test, we used the DBCSR (Distributed Blocked Compressed Sparse Row) algorithm included to take care of the sparse matrix-matrix multiplies. The DBCSR library is based on LibSMM, a small matrix matrix multiply library, which transforms the global sparse matrix multiplications into local small matrix matrix multiplies that are performed on the GPU. Therefore, even if the motif is matrix multiplication, the actual computations are memory and communication bound. 
We used the Titanium Dyoxide test case (TiO2) provided with the cude-enabled cp2k using 256 nodes, 1 MPI process per node, 8 threads per MPI process. Since one rack of XC-30 has at most 192 nodes, we ran two instances of the same test to cover most of the 3 cabinets available in order to compare with the cabinet-level PMDB query.
\begin{table}
\centering
\begin{tabular}{|l|rrr|}
\hline
TiO2       & PMDB (node) &  PMDB (rack) & External PM \\ 
Total Power (kW)       & 152.7 & 149.1 & 161.0 \\ 
Energy To Solution (kWh) & 5.21 & 5.05 & 5.50 \\
\hline
\end{tabular}
\caption{TiO2 benchmark results for CP2K using node-level and cabinet-level PMDB queries compared to the External Power Meter} 
\label{tbl:cp2k-results}
\end{table}
Tab. ($\ref{tbl:cp2k-results}$) shows the results for the TiO2 benchmark. We can see that the power consumption is significantly below that reported by the exeternal power meter. This can be explained by the very configuration of the Clogin and the test setup: since we used a square BLACS grid of 16 by 16 nodes, we had to duplicate the run twice to cover the three cabinets at our disposal. During the external power measurements, we had a problem with one of the power meters which reported an incorrect power measurement for the second cabinet so we used the same power consumption as the first, making the comparison a bit dodgy. However, all measurements are within 10%, which is still a good match.  

